FSMI: Fast computation of Shannon Mutual Information for information-theoretic mapping

Exploration tasks are embedded in many robotics applications, such as search and rescue and space exploration. Information-based exploration algorithms aim to find the most informative trajectories by maximizing an information-theoretic metric, such as the mutual information between the map and potential future measurements. Unfortunately, most existing information-based exploration algorithms are plagued by the computational difficulty of evaluating the Shannon mutual information metric. In this paper, we consider the fundamental problem of evaluating Shannon mutual information between the map and a range measurement. First, we consider 2D environments. We propose a novel algorithm, called the Fast Shannon Mutual Information (FSMI). The key insight behind the algorithm is that a certain integral can be computed analytically, leading to substantial computational savings. Second, we consider 3D environments, represented by efficient data structures, e.g., an OctoMap, such that the measurements are compressed by Run-Length Encoding (RLE). We propose a novel algorithm, called FSMI-RLE, that efficiently evaluates the Shannon mutual information when the measurements are compressed using RLE. For both the FSMI and the FSMI-RLE, we also propose variants that make different assumptions on the sensor noise distribution for the purpose of further computational savings. We evaluate the proposed algorithms in extensive experiments. In particular, we show that the proposed algorithms outperform existing algorithms that compute Shannon mutual information as well as other algorithms that compute the Cauchy-Schwarz Quadratic mutual information (CSQMI). In addition, we demonstrate the computation of Shannon mutual information on a 3D map for the first time.

==> 6_1_fsmi_rle.tex <==
% !TEX root = root_ijrr.tex

\section{Fast Shannon Mutual Information for 3D Environment using Run Length Encoding}
\label{sec:fsmi_3d}

An extension of a 2D occupancy map is a 3D voxel map~\citep{roth1989building, moravec1996robot}. However, such a data structure requires much more memory to store because of the additional dimension. Fortunately, in real world scenarios the 3D space that a robot navigates has structure: empty spaces are typically large and continuous. Taking advantage of this structure, researchers developed an adaptive data structured called OctoMap to compresses the map by using voxels of varying sizes. Large homogeneous regions that would contain thousands of small cells can be represented with a single cell in an OctoMap representation. Thus, OctoMaps have become widely used in 3D mapping and exploration algorithms~\citep{endres20143, whelan2015real, burri2015real}. Figure~\ref{fig:octomap_raytracing} presents an illustration of an OctoMap representation.

To the best of our knowledge, there has been no prior works discussing the computation of mutual information between range measurement and the environment on OctoMap. In this section, we show an extension of the FSMI method for such a map representations. It is based on direct computation on a compressed vector using run-length encoding (RLE)~\citep{robinson1967results}. The key idea behind the run-length encoding is to represent consecutive cells with the same values as one larger cell, which makes it a valuable compression method for large-scale maps with a reasonable degree of homogeneity. In particular, maps in three-dimensional spaces benefit from this compression method immensely.

This section is organized as follows. Section~\ref{sec:octomap_ray_tracing} discusses the OctoMap representation, which uses the run-length encoding to efficiently store and process three-dimensional maps. 
%
Section~\ref{sec:fsmi_rle_problem_statement} formalizes the problem of adapting FSMI to run-length encoding. Section~\ref{sec:fsmi_rle_tabulated} presents an efficient tabulation based solution. Section~\ref{sec:fsmi_rle_gaussian_truncation} discusses a numerical issue with the proposed solution and resolves it using Gaussian truncation. Finally, Section~\ref{sec:fsmi_rle_uniform} introduces a Uniform-FSMI algorithm for maps with run-length encoding.

\subsection{Ray-tracing on OctoMap}
\label{sec:octomap_ray_tracing}

\begin{figure}[!tb]
\centering 
\subfigure[Ray-tracing on OctoMap]{\label{fig:octomap_raytracing}\includegraphics[width=0.7\columnwidth]{figures/octomap/octo_ray_tracing.pdf}}
\subfigure[Ray-tracing result represented by run-length encoding (RLE)]{\label{fig:octomap_rle}\includegraphics[width=0.9\columnwidth]{figures/octomap/octo_RLE.pdf}}
\caption{An illustrative example of how an OctoMap representation adaptively represent an environment, and how ray-tracing on the OctoMap representation results in an occupancy sequence represented by run-length encoding (RLE) format}
\end{figure}

Ray-tracing on an OctoMap differs from the ray-tracing on a fixed-resolution voxel map by allowing a beam to intersect with cells of drastically different sizes. In addition, depending on the level of compression, the number of cells can also significantly vary along with the cell size. Recall that the Shannon mutual information does not distinguish the cells because of their sizes. As a consequence, the Shannon mutual information between a beam and $10$ small continuous cells of the same occupancy value will be significantly higher than the Shannon mutual information between the same beam and a merged cell that is 10$\times$ bigger. This means the Shannon mutual information couples with the compression strength. 


Hence, instead of measure the Shannon mutual information on a vector of cells with varying width, we propose to convert the vector into a vector of cells with uniform width and then measure the Shannon mutual information.

Figure~\ref{fig:octomap_raytracing} and Figure~\ref{fig:octomap_rle} illustrate how we achieve it. Specifically, let us assume that the ray-tracing algorithm returns $n_r$ cells. In space, the beam intersects enters the $i$-th intersected cell at $q_i$ and exists at $q_{i + 1}$. Suppose a 3D point $Q_i$ maps to a 1D point $q_i$ on the beam. Suppose the minimal size of the cell in an OctoMap is $w_0$. Then we transform the $i$-th cell from a big cell of length $q_{i + 1} - q_i$ to a group of cells of length $w_0$ with the number of cells being $L_i = \mathrm{round}((q_{i + 1} - q_i) / w_0)$. In this way, the variation of the number of cells due to the different compression levels is significantly reduced.

The outcome of this method is an occupancy sequence compressed by the run-length encoding (RLE) compression method. It is indeed possible to decode it into a normal occupancy vector and then apply the FSMI algorithm to compute Shannon mutual information. In the next section, we propose a new method that computes the Shannon mutual information computation directly on the compressed sequence. We show that its time complexity is linear in size of the compressed length vector, which translates to significant computational savings in practical problem instances. 

% -----------------------------------------------------------------------------------------------------
\subsection{FSMI on Occupancy Sequence compressed by Run-Length Encoding}
\label{sec:fsmi_rle_problem_statement}
% 
In this subsection, we formally present the algorithm to compute the Shannon mutual information between a sensor beam and an array of cells whose occupancy values are compressed by the run length encoding. Specifically, suppose the sequence consists of $n_r$ homogeneous groups of cells; the $i$-th group has $L_i\in \mathbb{Z}^{+}$ number of  cells of the same occupied probability $o_i\in(0, 1)$. The total number of cells, $n$, relates to $L_i$ by $\sum_{i=1}^{n_r} L_i = n$. This means the vector of occupancy values for the range measurement $O$ can be formally expressed as
\begin{equation}
\label{eqn:occup_rle}
O = \{\underbrace{o_1,\ldots, o_1}_{\textrm{repeated $L_1$ times}}, ..., \underbrace{o_n,\ldots, o_n}_{\textrm{repeated $L_n$ times}}\}.
\end{equation} 

For the $u$-th group of cells, let $s_u = \sum_{i < u} l_i$ be the index of the first cell. 

We further assume that the noise follows normal distribution of constant variance $\sigma^2$ regardless of the length of the beam. In addition, let us assume that each cell has same width $w_0$. The goal is to compute $I(M'; Z)$ where $M'$ are the occupancy cells the range measurement can intersect. Before stating the results, we define a few terms used throughout this section.

First, we let $P_E(u) = \prod_{i < u} (1-o_i)^{L_i}$ denote the probability that all the cells on the beam before the first cell of the $u$-th group of cells are all empty. We use the subscript $E$ from the word \emph{empty} to distinguish this term from the previously used $P(e_j)$, the probability of the $j$-th cell being the first non-empty cell in $M'$. In fact, we can use $P_E(u)$ to help the evaluation of $P(e_j)=o_j\prod_{l<j}(1-o_l)$ for the $j$-th cell if it falls into the $u$-th group of cells. Similarly, we define $D_E(u)=\sum_{i< u} L_i f(\delta_{emp}, r_i)$ to help the computation of $C_k = \sum_{l<k} f(\delta_{emp}, r_l) + f(\delta_{occ}, r_k)$ for the $k$-th cell if it belongs to the $u$-th group of cells. Both $P_E(u)$ for all $u\in \{1, \ldots, n_r\}$ and $D_E(u)$ for all $u\in\{1, \ldots, n_r\}$ can be computed in $O(n_r)$.

The following theorem states the main result of this section. 

To present the main result of this section, we define the following notation: Let $\bar{o}_u = 1-o_u$. Let $\sigma' = \sigma / w$. Let $G_{k, j} = \exp\left(-\frac{(k - j)^2}{2\sigma'^2}\right)$. Figure~\ref{fig:fsmi_rle_notation} illustrates these notations as well as the problem setup of the theorem.

\begin{theorem}[FSMI-RLE]
\label{theorem:group_fsmi_rle}
We have
\begin{equation}
\begin{split}
\label{eqn:group_fsmi_rle_exact}
&I(M; Z) = \sum_{u = 1}^{n_r}\sum_{v = 1}^{n_r} \frac{P_E(u) o_u}{\sqrt{2\pi}\sigma'}\Big(\\
&(D_E(v) + f(\delta_{occ}, r_v))\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} j\cdot \bar{o}_{u}^{j} G_{j + s_u, k + s_v} +  \\ 
& f(\delta_{emp}, r_v)) \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} \bar{o}_{u}^{j} G_{j + s_u, k + s_v} \Big).
\end{split}
\end{equation}
\end{theorem}

\begin{figure}[!tb]
\centering 
\includegraphics[width=0.9\columnwidth]{figures/octomap/fsmi_rle_setup.pdf}
\caption{Notations for FSMI computation on an occupancy sequence compressed by RLE.}
\label{fig:fsmi_rle_notation}
\end{figure}

\begin{proof}
We reorganize Eqn.~\eqref{eqn:fast_exact_mi} into double sum over groups of cells defined in Eqn.~\ref{eqn:occup_rle}:
\begin{equation}
\label{eqn:eqn_from_fsmi}
I(M; Z) = \sum_{u = 1}^{n_r} \sum_{v = 1}^{n_r} \sum_{j = 0}^{L_u - 1}\sum_{k = 0}^{L_v - 1} P(e_{s_u + j}) C_{s_v + k} G_{s_u + j, s_v + k}.
\end{equation}
For a fixed $u$, $\forall j$ we have
\begin{equation}
\label{eqn:p_e_u}
P(e_{s_u + j}) = P_E(u)(1-o_u)^{j}o_u.
\end{equation}
Similarly, 
\begin{equation}
\label{eqn:C_v}
C_{s_v + k} = D_E(v) + k\cdot f(\delta_{emp}, r_v) + f(\delta_{occ}, r_v).
\end{equation}
Substituting Eqn.~\eqref{eqn:p_e_u} and Eqn.~\eqref{eqn:C_v} into Eqn.~\eqref{eqn:eqn_from_fsmi} completes the proof.
\qed
\end{proof}

Let $t = s_u - s_v$. Thus, $G_{s_u + j, s_v + k} =  \exp\left(-\frac{(k + t - j)^2}{2\sigma'^2}\right)$.  Theorem~\ref{theorem:group_fsmi_rle} motivates us to study the two terms defined as follows. 

For notational simplicity, we define $x=1-o_u$; thus, $0<x<1$.

\begin{equation}
\begin{split}
\label{eqn:AB_original}
A[x, L_u, L_v, t] &= \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} x^j \exp{\left(-\frac{(j-k+t)^2}{2\sigma'^2}\right)}\\
B[x, L_u, L_v, t] &= \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} k\cdot x^j \exp{\left(-\frac{-(j-k+t)^2}{2\sigma'^2}\right)}.
\end{split}
\end{equation}

We would like to find an algorithms to evaluate $A[x, L_u, L_v, t]$ and $B[x, L_u, L_v, t]$ in $O(1)$ independent of the length of the range measurement and the occupancy map resolution.

In an exploration trial of a robot, the noise variance $\sigma^2$ remains constant; hence we do not consider it a parameter in the above two terms. Such $O(1)$ algorithms enable exact evaluation of $I(M; Z)$ in $O(n_r^2)$ instead of $O(n^2)$. Note that $n_r$ is significantly smaller than $n$ because of the run-length encoding compression. Hence, this reduction of complexity will translate to significant acceleration of mutual information computation in practice as long as the OctoMap achieves reasonable compression for the scene.


\subsection{Tabulated Solution}
\label{sec:fsmi_rle_tabulated}
Without approximation, we could not find closed-form solutions to the two terms in Eqn.~\eqref{eqn:AB_original}. With approximation, we are able to derive closed-form solutions to them. Unfortunately, these solutions are too complicated to be practical. Despite their $O(1)$ time complexity, evaluating them costs an overhead that far overshadows the reduction of the overall FSMI complexity from $O(n)$ to $O(n_r)$ by RLE compression. Appendix~\ref{sec:appendix_analytic} discusses these closed-form solutions in detail. Therefore, instead of computing $A$ and $B$ analytically with approximation, we employ a precomputed look-up table based approach for fast evaluation of $A$ and $B$. 

The tabulation strategy for $A$ and $B$ are similar. We start with the solution for $A[x, L_u, L_v, t]$. To enable tabulation, we first quantize $x$ onto a finite set of values $\mathcal{X}$ with uniform quantization over $[0, 1]$. We also enumerate $L_u, L_v, t$. Since $1\le L_u, L_v, t\le n$. Let $|\mathcal{X}|$ be the number of quantization levels for the occupancy value. 

\begin{lemma}[Size of the table for $A$ and $B$]
The number of entries in $A$ is $|\mathcal{X}| n^3$. The same is for $B$.
\end{lemma}



This rest of this section proposes a novel way to tabulate $A$ that drastically reduces the size of the table. Instead of tabulating $A[x, L_u, L_v, t]$, we propose to tabulate $\alpha[x, L_u, L_v] = \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} x^j \exp{\left(-\frac{(j-k)^2}{2\sigma'^2}\right)}$. Then from $\alpha[x, L_u, L_v]$ we can easily compute $A[x, L_u, L_v, t]$ according to the following lemma.

\begin{lemma}
\label{lemma:A_and_alpha}
When $t \ge 1$, 
\begin{equation}
\label{eqn:alpha_tab_pos_t}
A[x, L_u, L_v, t] = x^{-t}\left(\alpha[x, L_u + t, L_v] - \alpha[x, t, L_v]\right).
\end{equation}
When $t \le -1$,
\begin{equation}
\label{eqn:alpha_tab_zero_t}
A[x, L_u, L_v, t] = \left(\alpha[x, L_u, L_v - t] - \alpha[x, L_u, -t]\right).
\end{equation}
When $t = 0$,
\begin{equation}
\label{eqn:alpha_tab_neg_t}
A[x, L_u, L_v, t] = \alpha[x, L_u, L_v].
\end{equation}
\end{lemma}

\begin{proof}
When $t\ge 1$, 
\begin{equation}
\begin{split}
    &A[x, L_u, L_v, t] = \sum_{j = 0}^{L_u - 1}\sum_{k = 0}^{L_v - 1} x^{j} \exp\left(-\frac{(j + t - k)^2}{2}\right)\\
    =& \sum_{j = 0}^{L_u - 1}\sum_{k = 0}^{L_v - 1} x^{-t}x^{j + t} \exp\left(-\frac{(j + t - k)^2}{2}\right)\\
    =&x^{-t}\sum_{j = 0}^{L_u - 1}\sum_{k = 0}^{L_v - 1} x^{j + t} \exp\left(-\frac{(j + t - k)^2}{2}\right)\\
    =&x^{-t}\sum_{j = t}^{L_u + t - 1}\sum_{k = 0}^{L_v - 1} x^j \exp\left(-\frac{(j - k)^2}{2}\right)\\
    =&x^{-t}\left(\alpha[x, L_u + t, L_v] - \alpha[x, t, L_v]\right).
\end{split}
\end{equation}

Similarly, when $t\le -1$,
\begin{equation}
\begin{split}
    &A[x, L_u, L_v, t] = \sum_{j = 0}^{L_u - 1}\sum_{k = 0}^{L_v - 1} x^{j} \exp\left(-\frac{(j + t - k)^2}{2}\right)\\
    =& \sum_{j = 0}^{L_u - 1}\sum_{k = -t}^{L_v - t - 1} x^{j} \exp\left(-\frac{(j - k)^2}{2}\right)\\
    =&\alpha[x, L_u, L_v - t] - \alpha[x, L_u, -t].
\end{split}
\end{equation}
\qed
\end{proof}

According to this lemma, evaluating an entry in $A$ requires two access of entries in $\alpha$ and simple arithmetic operations. If we do not even want to compute $x^{-t}$, we can maintain a very small look-up table for it since $x$ has been quantized.

\begin{lemma}[Size of table for $\alpha$]
\label{lemma:alpha_table_size}
$\alpha[x, L_u, L_v]$ needs to have $|\mathcal{X}|n^2$ entries to reconstruct any entry of $A[x, L_u, L_v, t]$ where $L_u$, $L_v$ and $t = s_u - s_v$ are from Eqn.~\eqref{eqn:group_fsmi_rle_exact}.
\end{lemma}

\begin{proof}
First, $|t| = |s_u - s_v|\le max(s_u, s_v) \le n$. When $t\ge 1$, $L_u + t = L_u + s_u - s_v = L_u + \sum_{i = v}^{u - 1} L_i = \sum_{i = v}^{u} L_i \le n$. Similarly, when $t \le -1$, $Lv - t = L_v - s_u + s_v = L_v + \sum_{i = u}^{v - 1} L_i = \sum_{i = u}^{v} L_i\le n$. 

Therefore, all the indexes for $\alpha$ in Eqn.~\eqref{eqn:alpha_tab_pos_t}\eqref{eqn:alpha_tab_zero_t}\eqref{eqn:alpha_tab_neg_t} are bounded within $[1, n]$. The case for $t = 0$ is trivial.

Hence the computation for $A[x, L_u, L_v, t]$ involves at most $|\mathcal{X}|n^2$ entries in $\alpha$.
\qed
\end{proof}


Note that the Lemma \ref{lemma:alpha_table_size} does not state the sufficiency of $\alpha$ for $A$ for general $1\le L_u, L_v, t\le n$ not from Eqn.~\eqref{eqn:group_fsmi_rle_exact}. In fact, to support the computation of $A$ for general $L_u, L_v, t$ the size of the table for $\alpha$ needs to be four times larger.

We can incrementally build $\alpha[x, L_u, L_v]$ according to the following lemma:

\begin{lemma}[Incremental construction of $\alpha$] 
\label{lemma:alpha_build}
The base value is $\alpha[x, 1, 1] = 1$.

When $L_u > 1$ and $L_v > 1$
\begin{equation}
\begin{split}
\alpha[x, L_u, L_v] =& \alpha[x, L_u - 1, L_v] + \alpha[x, L_u, L_v - 1] -\\
&\alpha[x, L_u - 1, L_v - 1] + \\
&x^{L_v - 1} \exp{\left(-\frac{(L_u - L_v)^2}{2\sigma'^2}\right)}.
\end{split}
\end{equation}.
When $L_u = 1, L_v > 1$, 
\begin{equation}
\alpha[x, L_u, L_v] = \alpha[x, L_u, L_v - 1] + x^{L_v - 1} \exp{\left(-\frac{(1 - L_v)^2}{2\sigma'^2}\right)}. 
\end{equation}.
When $L_u > 1, L_v = 1$, 
\begin{equation}
\alpha[x, L_u, L_v] = \alpha[x, L_u - 1, L_v ] + \exp{\left(-\frac{-(L_u - 1)^2}{2\sigma'^2}\right)}.
\end{equation}
\end{lemma}

Each entry of the table takes $O(1)$ time to fill. Therefore, the time complexity to fill $\alpha[x, L_u, L_v]$ is $O(|\mathcal{X}|N^2)$. 

Similarly, instead of tabulating $B[x, L_u, L_v, t]$, we propose to tabulate $\beta[x, L_u, L_v] = \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} k\cdot x^j \exp{\left(-\frac{(j-k)^2}{2\sigma'^2}\right)}$. Given $\beta$, we can compute $B[x, L_u, L_v, t]$ in $O(1)$ according to the following lemma

\begin{lemma}
\label{lemma:B_and_beta}
When $t \ge 1$, 
\begin{equation}
B[x, L_u, L_v, t] = x^{-t}\left(\beta[x, L_u + t, L_v] - \beta[x, t, L_v]\right).
\end{equation}
When $t \le -1$,
\begin{equation}
\begin{split}
B[x, L_u, L_v, t] =& \beta[x, L_u, L_v - t] - \beta[x, L_u, -t] + \\
&t\cdot A[x, L_u, L_v, t].
\end{split}
\end{equation}
When $t = 0$,
\begin{equation}
B[x, L_u, L_v, t] = \beta[x, L_u, L_v].
\end{equation}
\end{lemma}

\begin{proof}
The case for $t = 0$ is trivial. The case for $t\ge 1$ is almost the same as Lemma~\ref{lemma:A_and_alpha}. When $t\le 1$, we have

\begin{equation}
\begin{split}
&B[x, L_u, L_v, t] = \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} k\cdot x^j \exp{\left(-\frac{(j + t -k)^2}{2\sigma'^2}\right)}\\
=&\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} (k - t + t)\cdot x^j \exp{\left(-\frac{(j + t - k)^2}{2\sigma'^2}\right)}\\
=&\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} (k - t)\cdot x^j \exp{\left(-\frac{(j-(k - t))^2}{2\sigma'^2}\right)} +\\
&\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} t\cdot x^j \exp{\left(-\frac{(j+ t - k)^2}{2\sigma'^2}\right)}\\
= &\sum_{j=0}^{L_u - 1}\sum_{k=-t}^{L_v-t - 1} k\cdot x^j \exp{\left(-\frac{(j-k)^2}{2\sigma'^2}\right)} +\\
&\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} t\cdot x^j \exp{\left(-\frac{(j+ t - k)^2}{2\sigma'^2}\right)}\\
= &\beta[x, L_u, L_v - t] - \beta[x, L_u, - t] + t\cdot A[x, L_u, L_v, t]
\end{split}
\end{equation}.
\qed
\end{proof}

Note that when $t \le -1$, the evaluation of $B[x, L_u, L_v, t]$ depends on $A[x, L_u, L_v, t]$. This motivates us to always evaluate $A[x, L_u, L_v, t]$ before $B[x, L_u, L_v, t]$.

The size of the table $\beta$ is the same as the size of the table $\alpha$.


\subsection{Fixing Numerical Issues via Gaussian Truncation}
\label{sec:fsmi_rle_gaussian_truncation}
Unfortunately, the above procedure suffers from intrinsic numerical issues. In 3D OctoMap there can be large homogeneous regions such as big empty space. When a sensor beam intersect with such region, the output occupancy sequence can have a long segment of homogeneous cells. Without loss of generality, let us call the group of cell $v$, and the number of cells in this group, $L_v$, is large. The existence of such cell group causes numerical issues for the evaluation of $A[\bar{o}_u, L_u, L_v, t]$ with Eqn.~\eqref{eqn:alpha_tab_pos_t} when $\exists u, u > v$ and $L_u$ is also big.

Specifically, according to Eqn.~\eqref{eqn:alpha_tab_pos_t}, $A[\bar{o}_u, L_u, L_v, t]$ is the product of $\left(\bar{o}_u\right)^{-t}$ and $\alpha[\bar{o}_u, L_u + t, L_v] - \alpha[\bar{o}_u, t, L_v]$. Note that $t = s_u - s_v \ge L_v$. Therefore, $t$ is also very large. When $\bar{o}_u$ is close to $0$,$\bar{o}_u^{-t}$ becomes astronomically big. At the same time $\left(\alpha[\bar{o}_u, L_u + t, L_v] - \alpha[\bar{o}_u, t, L_v]\right)$ becomes extremely small. If there is infinite precision, the multiplication of these two terms should neutralize each other. Unfortunately, we incrementally compute $\alpha[\bar{o}_u, L_u + t, L_v]$ from $\alpha[\bar{o}_u, t, L_v]$ according to Lemma.~\ref{lemma:alpha_build} as follows:
\begin{equation}
\begin{split}
\alpha[\bar{o}_u, L_u + t, L_v] &= \alpha[\bar{o}_u, t, L_v] + \\
&\sum_{i = t + 1}^{L_u + t} (1-o_u)^{i - 1} \exp{\left(-\frac{(i -L_v)^2}{2\sigma'^2}\right)}.
\end{split}
\end{equation}

When $i > t$, $(1-o_u)^{i - 1}$ is negligibly small compared with $\alpha[x, t, L_v]$. Therefore, accumulating $(1-o_u)^{i - 1}, t + 1\le i\le L_u + t$ on top of $\alpha[x, t, L_v]$ to compute $\alpha[x, L_u + t, L_v]$ introduces significant loss of precision, which passes on to $\alpha[x, L_u + t, L_v] - \alpha[x, t, L_v]$. Consequentially, $\alpha[x, L_u + t, L_v] - \alpha[x, t, L_v]$ can no longer neutralize the big number $\bar{o}_u^{-t}$ in the product. In practice, we frequently observe the multiplication to be an erroneously large number, corrupting the whole computation.

We believe that this problem is intrinsic to the proposed tabulation method with $\alpha$ and $\beta$. The original algorithm that directly tabulates $A$ and $B$ does not suffer from this issue. The cost is two orders of magnitude larger memory requirement.

We find that the key to fix the numerical issue is to prevent $t$ from being too big. Therefore, the Gaussian truncation technique can serve this purpose. A side benefit is further reduction of the size of the look-up tables $\alpha$ and $\beta$, making the algorithm memory friendly to extremely memory constrained platforms such as FPGA and ASIC.

Recall that the Gaussian truncation set $G_{k, j}$ to $0$ when $|k-j| > \Delta$ where $\Delta$ is a constant as small as $3$ or $5$. Applying this truncation to the FSMI-RLE algorithm summarized in Eqn.~\eqref{eqn:group_fsmi_rle_exact} can have different impact on the accumulated terms according the relative spatial location and the length of two groups of cells $u$ and $v$. At a high level, the impact can be

\begin{itemize}
    \item[Case 1] The two groups are two far away from each other. All terms are truncated
    \item[Case 2] The two groups are small and close to each other. No term is truncated.
    \item[Case 3] Some terms are truncated to $0$ while others remain the same.
\end{itemize}

In case 1, $A[x, L_u, L_v, t] = B[x, L_u, L_v, t] = 0$; hence, we can simply skip the pair $(u, v)$ in the summation. We formalize the condition for this case to happen in the following lemma:

\begin{lemma}[Zero Mutual Information Blocks after Gaussian Truncation]
\label{lemma:zero_blocks_truncation}
If $G_{k, j} = 0$ when $|k - j| > \Delta$, then $A[x, L_u, L_v, t] = 0$ if and only if $t > 0, t - L_v + 1 > \Delta$ or $t < 0, -t - L_u + 1 > \Delta$.\end{lemma}

\begin{proof}
Note that $G_{j + s_u, k + s_v} = 0$ when $|j + s_u - k - s_v| > \Delta$. If $t> 0$ and $u > v$, we have $j + s_u > k + s_v$; thus, the condition transforms into $j - k + t > \Delta$. This needs to hold $\forall j\in[L_u - 1], \forall k\in[L_v - 1]$. Hence we need $(\min_{j, k} j - k + t) > \Delta$. This is equivalent to $t - L_v + 1 > \Delta$.

The argument for the case of $u < v$ is the similar, so we skip it.
\qed
\end{proof}

\begin{figure}[!tb]
\centering{
\includegraphics[width= \columnwidth]{figures/octomap/gaussian_truncation.pdf}
}
\caption{When the condition in Lemma~\ref{lemma:zero_blocks_truncation} holds, Gaussian truncation sets the Shannon mutual information contribution between these two blocks to zero.}
\label{fig:block_truncation}
\end{figure}

Figure~\ref{fig:block_truncation} illustrates this lemma. It enables us to skip computations for a pair of $(u, v)$. However, it alone is not enough to fix the numerical issue since it cannot filter out two adjacent large blocks of cells, so $L_v$ can still be big.

The condition for case 2 to happen is summarized below:
\begin{lemma}[Condition of no impact from Gaussian Truncation]
\label{lemma:zero_blocks_truncation_no_impact}
If $G_{k, j} = 0$ when $|k - j| > \Delta$, then $A[x, L_u, L_v, t]$ is not changed if and only if $t > 0, \Delta \ge t + L_u - 1$ or $t < 0, \Delta + t\ge L_v - 1$ or $t = 0, L_u\le \Delta$\end{lemma}

The proof of this lemma is almost the same as the proof for \ref{lemma:zero_blocks_truncation}.

Case 3 is more complicated. After the truncation, the start of the block and the length of the block can both change. The following lemma describes the new start and the length of the block:

\begin{lemma}[Start position and the length of the new blocks after truncation]
\label{lemma:start_length_truncation}
If $u > v$, i.e., $t > 0$, $s_v' = \max{(s_v, s_u - \Delta)}$, $L_v' = s_v + L_v - s_v'$, $s_u' = s_u$ and $L_u' = s_v + L_u - 1 + \Delta - s_u$. If $u < v$, i.e., $t < 0$, $s_u' = \max{(s_u, s_v - \Delta)}$, $L_u' = s_u + L_u - s_u'$, $s_v' = s_v$ and $L_v' = s_u + L_v - 1 + \Delta - s_v$.
\end{lemma}

Figure~\ref{fig:truncation_position} visually illustrates this lemma.

\begin{figure}[!tb]
\centering{
\includegraphics[width= 0.9\columnwidth]{figures/octomap/gaussian_truncation_sub.pdf}
}
\caption{Gaussian Truncation can change the start and the length of a block of cell.}
\label{fig:truncation_position}
\end{figure}

\begin{theorem}[Truncation fixes the numerical issue]
If $G_{k, j} = 0$ when $|k - j| > \Delta$, if $u\ne v$, we have
\begin{equation}
L_u'\le \Delta, L_v'\le \Delta.    
\end{equation}

\end{theorem}

\begin{proof}
If $u < v$, we have
\begin{equation}
\begin{split}L_u' = &s_u + L_u - 1 - \max{(s_u, s_v - \Delta)}  + 1 \\
\le& s_u + L_u - 1 - s_v + \Delta + 1 \\
\le&\Delta.
\end{split}
\end{equation}

The last step holds because $s_v - s_u \ge L_u$.
Similarly,

\begin{equation}
\begin{split}
L_v' =& \min{(s_u + L_u - 1 + \Delta, s_v + L_v - 1)} - s_v + 1\\ 
\le& s_u + L_u - 1 + \Delta - s_v + 1\\
\le& \Delta.
\end{split}
\end{equation}
Since $|t'| = |s_v' - s_u'|\le \Delta$, $L_u' + |t'|\le 2\Delta$ and $L_v' + |t'|\le 2\Delta$.

Because of the symmetry, the conclusions also hold for the case of $u > v$.
\qed
\end{proof}

Bounding $L_u$ and $L_v$ within $\Delta$ resolves the numerical issue from the previous subsection. 
\begin{lemma}[Table size after truncation]
\label{lemma:alpha_beta_size_after_truncation}
After truncation, the size of $\alpha$ and $\beta$ are both $4|\mathcal{X}|\Delta^2$.
\end{lemma}
\begin{proof}
When $u\ne v$, let $t' = s_v' - s_u'$, we have $L_u' + |t| \le 2\Delta$ and $L_v + |t| \le 2\Delta$. Therefore, the second and third dimension of $\alpha$ and $\beta$ in Lemma~\ref{lemma:A_and_alpha} and Lemma~\ref{lemma:B_and_beta} when $t\ne 0$ are both bounded by $2\Delta$. \qed
\end{proof}



When $t = 0$, the start location and the length of the block remains the same after Gaussian truncation. Since numerical issues only happen when $t > 1$, we can safely keep the original algorithm for this case.

If we trim $\alpha$ and $\beta$ according to Lemma~\ref{lemma:alpha_beta_size_after_truncation},  we also remove $\alpha[x, L, L]$ and $\beta[x, L, L]$ where $L > 2\Delta$. Unfortunately, these terms are needed to compute compute $A[x, L_u, L_u, 0]$ and $B[x, L_u, L_u, 0]$ when $t = 0$. To address this, we introduce two additional tables $\theta[x, L] = \alpha[x, L, L]$ and $\gamma[x, L] = \beta[x, L, L]$ for store $\alpha[x, L, L]$ and $\beta[x, L, L]$. Each table introduces at most $|\mathcal{X}|\max_u {L_u}$ entries. 

It is worth noting that truncation changes the beginning of a group of cell as well as the length. Consequentially, we need to update the value of $P_E(u)$ and $D_E(u)$ separately for each pair $(u, v)$. Those modifications are summarized into the following theorem:

\begin{theorem}[Approx-FSMI-RLE]
Suppose $s_u, L_u, s_v, L_v$ are truncated into $s_u'(u, v), L_u'(u, v), s_v'(u, v), L_v'(u, v)$ according to Lemma~\ref{lemma:start_length_truncation}. Let $\mathcal{V}_u$ be the set of indexes $u$ such that Gaussian Truncation would not set the term to $0$. Then the Shannon mutual information becomes
\begin{equation}
\begin{split}
\label{eqn:approx_fsmi_rle}
&I(M; Z) = \sum_{u = 1}^{n_r}\sum_{v\in \mathcal{V}_u, v\ne u} \frac{P_E(u) (1-o_u)^{L_u - L_u'(u, v)} o_u}{Z}\Big(\\
&(D_E(v) + (L_v - L_v'(u, v))f(\delta_{emp}, r_v) + \\
&f(\delta_{occ}, r_v)) A[x, L_u'(u, v), L_v'(u, v), t] + \\
& f(\delta_{emp}, r_v)) B[x, L_u'(u, v), L_v'(u, v), t] \Big) + \\
& \sum_{u = 1}^{n_r} \frac{P_E(u)o_u}{Z}(D_E(u) + f(\delta_{occ}, r_v))\theta[x, L_u] + \\
& f(\delta_{emp}, r_u)) \gamma[x, L_u]\Big).
\end{split}
\end{equation}
\end{theorem}

\begin{proof}
The proof follows Theorem~\ref{theorem:group_fsmi_rle}. After the Gaussian truncation, we update the value of $P_E'(u)$ when $s_u'\ne s_u$ and  $D_E'(v)$ when $s_v'\ne s_v$. Specifically, when $L_u'\ne L_u$, 
\begin{equation}
\label{eqn:group_fsmi_truncation_P_E}
\begin{split}
    P_E'(u) &= P_E(u)(1-o_u)^{s_u(u, v)' - s_u}\\
    &= P_E(u)(1-o_u)^{L_u(u, v) - L_u'(u, v)}.
\end{split}
\end{equation}
When $L_v'\ne L_v$, 
\begin{equation}
\label{eqn:group_fsmi_truncation_D_E}
D_E'(v) = D_E(v) + (L_v - L_v'(u, v))f(\delta_{emp}, r_v).
\end{equation}
Substituting Eqn.~\eqref{eqn:group_fsmi_truncation_P_E} and ~\eqref{eqn:group_fsmi_truncation_D_E} into Eqn.~\eqref{eqn:group_fsmi_rle_exact} and separate the case of $u\ne v$ from the case of $u=v$, we get Eqn.~\eqref{eqn:approx_fsmi_rle}. \qed
\end{proof}

The complete algorithm is summarized in Algorithm~\ref{alg:approx_fsmi_rle}.

\begin{theorem}[Complexity of the Approx-FSMI-RLE algorithm]
The complexity of Algorithm~\ref{alg:approx_fsmi_rle} is $O(\Delta n_r)$.
\end{theorem}

The previous theorem holds because $|\mathcal{V}_u|\le (2\Delta + 1)$ in Algorithm~\ref{alg:approx_fsmi_rle}. Since $\Delta$ is a constant as small as $5$ regardless of $n_r$, the algorithm essentially scales linearly with respect to $n_r$ only.

% ---------------------------------------------------------------------------
% P_E_u
\begin{algorithm}[!tb]
\caption{Evaluate $P_E(u)$ for $1 \le u \leq n_r$}\label{alg:P_E_u}
\begin{algorithmic}[1]
\Require $o_u$, $L_u$ for $1 \leq u \leq n_r$
\State $P_E(1)\leftarrow 1$
\For{$u=2$ \textbf{to} $n_r$}
    \State $P_E(u)\leftarrow P_E(u - 1)(1-o_{u - 1})^{L_{u - 1}}$
\EndFor
\State \Return $P_E(u)$ for $1\le u\le n_r$
\end{algorithmic}
\end{algorithm}
% ---------------------------------------------------------------------------
% D_E_v
\begin{algorithm}[!tb]
\caption{Evaluate $D_E(v)$ for $1 \le v \leq n_r$}\label{alg:D_E_v}
\begin{algorithmic}[1]
\Require $r_v$, $L_v$ for $1 \leq v \leq n_r$
\State $D_E(1)\leftarrow 0$
\For{$v=2$ \textbf{to} $n_r$}
    \State $D_E(v)\leftarrow D_E(v - 1) + L_{v - 1}f(\delta_{emp}, r_{v - 1})$
\EndFor
\State \Return $D_E(v)$ for $1\le v\le n_r$
\end{algorithmic}
\end{algorithm}
% ---------------------------------------------------------------------------
\begin{algorithm}[!tb]
\caption{The Approx-FSMI-RLE algorithm}\label{alg:approx_fsmi_rle}
\begin{algorithmic}[1]
\Require Noise standard derivation $\sigma$, cell width $w$ and $L_i, o_i, r_i$ for $1\le i\le n_r$, quantization resolution $o_{res}$, Gaussian truncation width $\Delta$.
\State $I\leftarrow 0$
\State $\sigma' = \sigma / w$

\State Compute $P_E(u)$ for $1\leq j \leq n$ with Algorithm~\ref{alg:P_E_u}.
\State Compute $D_E(v)$ for $1 \leq k \leq n$ with Algorithm~\ref{alg:D_E_v}.
\State Tabulate $\alpha[x, L_u, L_v]$ and $\theta[x, L_u]$ with Algorithm~\ref{alg:tab_alpha_theta}.
\State Tabulate $\beta[x, L_u, L_v]$ and $\gamma[x, L_u]$ with Algorithm~\ref{alg:tab_beta_gamma}.
\For{$u=1$ \textbf{to} $n_r$}
    \State $x\leftarrow \mathrm{floor}((1-o_u) / o_{res})o_{res}$
	\For{$v\in \mathcal{V}_u$}
	    \If{$u=v$} 
	        \State $I\leftarrow I + P_E(u)o_u{Z}(D_E(u) + f(\delta_{occ}, r_v))\theta[x, L_u] + 
 f(\delta_{emp}, r_u)) \gamma[x, L_u]$
        \ElsIf{$u < v$ \textrm{ and } $s_u + L_u - 1 + \Delta \ge s_v$} 
            
            \State $s_u' \leftarrow \max{(s_u, s_v - \Delta)}$
            \State $L_u' \leftarrow s_u + L_u - s_u'$
            \State $s_v' \leftarrow s_v$
            \State $L_v' \leftarrow s_u + L_v - 1 + \Delta - s_v$
            \State $t\leftarrow s_u' - s_v'$
            \State $A = \left(\alpha[x, L_u', L_v' - t] - \alpha[x, L_u', -t]\right)$
            \State $B = \beta[x, L_u', L_v' - t] - \beta[x, L_u', -t] + t\cdot A$
            \State $I\leftarrow I + P_E(u) (1-o_u)^{L_u - L_u'(u, v)} o_u((D_E(v)  + f(\delta_{occ}, r_v)) A + f(\delta_{emp}, r_v)) B)$
        \ElsIf{$u > v$ \textrm{ and } $s_v + L_v - 1 + \Delta \ge s_u$}
            \State $s_v' \leftarrow \max{(s_v, s_u - \Delta)}$
            \State $L_v' \leftarrow s_v + L_v - s_v'$
            \State $s_u' \leftarrow s_u$
            \State $L_u' \leftarrow s_v + L_u - 1 + \Delta - s_u$
            \State $t\leftarrow s_u' - s_v'$
            \State $A = x^{-t}\left(\alpha[x, L_u' + t, L_v'] - \alpha[x, t, L_v']\right)$
            \State $B = x^{-t}\left(\beta[x, L_u' + t, L_v'] - \beta[x, t, L_v']\right)$
            \State $I\leftarrow I + P_E(u) o_u((D_E(v)  + f(\delta_{occ}, r_v)) A + (L_v - L_v'(u, v))f(\delta_{emp}, r_v) + f(\delta_{emp}, r_v)) B)$
        \EndIf
	\EndFor
\EndFor
\State $I\leftarrow I / (\sqrt{2\pi}\sigma')$
\State \Return $I$
\end{algorithmic}
\end{algorithm}


% ---------------------------------------------------------------------------
% Tabulating the algorithm
\begin{algorithm}[!tb]
\caption{Tabulating $\alpha[x, L_u, L_v]$ and $\theta[x, L_u]$}
\label{alg:tab_alpha_theta}
\begin{algorithmic}[1]
\Require $x_{res}$, $\sigma'$, $L_{bound}$, $L_{max}$
\State $N_x\leftarrow \mathrm{floor}(1 / x_{res})$
\For{$i = 0$ \textbf{to} $N_x$}
    \State $x\leftarrow i\cdot x_{res}$
    \State $\alpha[x, 1, 1] \leftarrow 1$
    \For{$L_u = 2$ \textbf{to} $L_{bound}$}
        \State $\alpha[x, L_u, 1] = \alpha[x, L_u - 1, 1] + \exp{(-\frac{(L_u - 1)^2}{2\sigma'^2})}$
    \EndFor
    
    \For{$L_v = 2$ \textbf{to} $L_{bound}$}
        \State $\alpha[x, 1, L_v] = \alpha[x, 1, L_v - 1] + x^{L_v - 1}\exp{(-\frac{(1 - L_v)^2}{2\sigma'^2})}$
    \EndFor
    
    \For{$L_u = 2$ \textbf{to} $L_{bound}$}
        \For{$L_v = 2$ \textbf{to} $L_{bound}$}
            \State $\alpha[x, L_u, L_v] = \alpha[x, L_u, L_v - 1] + \alpha[x, L_u - 1, L_v] - \alpha[x, L_u - 1, L_v - 1] + x^{L_v - 1}\exp{(-\frac{(L_u - L_v)^2}{2\sigma'^2})}$
        \EndFor
    \EndFor
    
    \For{$L = 1$ \textbf{to} $L_{bound}$}
        \State $\theta[x, L] = \alpha[x, L, L]$
    \EndFor
    
    \For{$L = L_{bound} + 1$ \textbf{to} $L_{\max}$}
        \State $\theta[x, L] \leftarrow \theta[x, L - 1]$
        \For{$i = 1$ \textbf{to} $L - 1$}
            \State $\theta[x, L] \leftarrow \theta[x, L] + x^{L- 1}\exp{(-\frac{(i - L)^2}{2\sigma'^2})}$
            \State $\theta[x, L] \leftarrow \theta[x, L] + x^{i- 1}\exp{(-\frac{(i - L)^2}{2\sigma'^2})}$
        \EndFor
        \State $\theta[x, L] \leftarrow \theta[x, L] + x^{L- 1}$
    \EndFor
\EndFor

\State \Return $\alpha$ and $\theta$
\end{algorithmic}
\end{algorithm}
% ---------------------------------------------------------------------------
% Tabulating the algorithm for $\beta, \gamma$

\begin{algorithm}[!tb]
\caption{Tabulating $\beta[x, L_u, L_v]$ and $\gamma[x, L_u]$}
\label{alg:tab_beta_gamma}
\begin{algorithmic}[1]
\Require $x_{res}$, $\sigma'$, $L_{bound}$, $L_{max}$
\State $N_x\leftarrow \mathrm{floor}(1 / x_{res})$
\For{$i = 0$ \textbf{to} $N_x$}
    \State $x\leftarrow i\cdot x_{res}$
    \State $\beta[x, 1, 1] \leftarrow 0$
    \For{$L_u = 2$ \textbf{to} $L_{bound}$}
        \State $\beta[x, L_u, 1] \leftarrow 0$
    \EndFor
    
    \For{$L_v = 2$ \textbf{to} $L_{bound}$}
        \State $\beta[x, 1, L_v] = \beta[x, 1, L_v - 1] + (L_v - 1)\exp{(-\frac{(1 - L_v)^2}{2\sigma'^2})}$
    \EndFor
    
    \For{$L_u = 2$ \textbf{to} $L_{bound}$}
        \For{$L_v = 2$ \textbf{to} $L_{bound}$}
            \State $\beta[x, L_u, L_v] = \beta[x, L_u, L_v - 1] + \beta[x, L_u - 1, L_v] - \beta[x, L_u - 1, L_v - 1] + (L_v - 1)x^{L_u - 1}\exp{(-\frac{(L_u - L_v)^2}{2\sigma'^2})}$
        \EndFor
    \EndFor
    
    \For{$L = 1$ \textbf{to} $L_{bound}$}
        \State $\gamma[x, L] = \beta[x, L, L]$
    \EndFor
    
    \For{$L = L_{bound} + 1$ \textbf{to} $L_{\max}$}
        \State $\gamma[x, L] \leftarrow \gamma[x, L - 1]$
        \For{$i = 1$ \textbf{to} $L - 1$}
            \State $\gamma[x, L] \leftarrow \gamma[x, L] + (i - 1)x^{L- 1}\exp{(-\frac{(i - L)^2}{2\sigma'^2})}$
            \State $\gamma[x, L] \leftarrow \gamma[x, L] + (L - 1)x^{i- 1}\exp{(-\frac{(i - L)^2}{2\sigma'^2})}$
        \EndFor
        \State $\gamma[x, L] \leftarrow \gamma[x, L] + (L - 1)x^{L- 1}$
    \EndFor
\EndFor

\State \Return $\beta$ and $\gamma$
\end{algorithmic}
\end{algorithm}



==> 6_2_uniform_fsmi_rle.tex <==
% !TEX root = root_ijrr.tex

% ------------------------------------------------------------------------------------------
\subsection{Uniform FSMI on Occupancy Sequence Compressed by Run-Length Encoding (RLE)}
\label{sec:fsmi_rle_uniform}
The Approx-FSMI-RLE algorithm assumes Gaussian distribution for the noise model. Section~\ref{sec:fsmi_uniform} shows how assuming uniform distribution for the noise model can simplify the FSMI algorithm in both time complexity and speed in practice. Unfortunately, the same benefit from the uniform distribution will not transfer to the FSMI on the occupancy sequence compressed by RLE. The FSMI algorithm with uniform noise has the same complexity as the Gaussian noise, and its speed in practice does not outperform Approx-FSMI-RLE either. We include the discussion only for the purpose of completion.

% Problem statement, main theoretic results
The setup of the problem is exactly the same as the Gaussian case except the noise model, which is formalized in Theorem~\ref{theorem:uniform_fsmi}.  Therefore, this section will follow the notation in Section~\ref{sec:fsmi_3d}, \eg, the distribution of the measurement noise is
\begin{equation}
P(Z | e_i) \sim U[l_i - H\Delta L,\; l_{i + 1} + H\Delta L],
\end{equation}
for $H\in\mathbb{Z}^+$. In addition, let $\mathbbm{1}(\cdot)$ be the indicator function. The following theorem presents the main result: 

\begin{theorem}[Uniform-FSMI-RLE]
, then
\begin{equation}
\begin{split}\label{eqn:group_uniform_fsmi_rle}
&I(M'; Z) = \sum_{u = 1}^{n_r}\sum_{v = 1}^{n_r} \frac{P_E(u) o_u}{2H + 1}\Big(\\
&(D_E(v) + f(\delta_{occ}, r_v))\sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} k\cdot \bar{o}_{u}^{j} \mathbbm{1}(|j + t - k)|\le H)\\ 
&+ f(\delta_{emp}, r_v)) \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} \bar{o}_{u}^{j}\mathbbm{1}(|j + t - k|\le H) \Big).
\end{split}
\end{equation}
\end{theorem}

This motivates us to focus on the computation of the following two terms:

\begin{equation}
\begin{split}
F[x, L_u, L_v, t] &= \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} x^j \mathbbm{1}(|j + t - k)|\le H)\\
G[x, L_u, L_v, t] &= \sum_{j=0}^{L_u - 1}\sum_{k=0}^{L_v - 1} k\cdot x^j \mathbbm{1}(|j + t - k)|\le H).
\end{split}
\end{equation}

The fastest way to compute these two terms is still tabulation. Essentially we can apply the same tabulation techniques in the Gaussian case to tabulate $F$ and $G$. However, the size of the resulting look-up table will be at least as big as the Gaussian case. In addition, the way that Eqn.~\ref{eqn:group_uniform_fsmi_rle} computes the Shannon mutual information with the two look-up tables is basically the same as Eqn.~\ref{eqn:group_fsmi_rle_exact}. Moreover, the uniform distribution itself serves as a truncation, very similar to Gaussian Truncation; it no longer activates the integration image trick on the uncompressed sequence. Therefore, the complexity of the uniform case is $O(n_rH)$, not lower than the Gaussian case $O(n\Delta)$. The computation speed of the Uniform-FSMI-RLE algorithm will NOT outperform the Approx-FSMI-RLE algorithm, either. Hence, we do not expand the details of the Uniform-FSMI-RLE algorithm.


